Finite-temperature transport in one-dimensional quantum lattice models

The last decade has witnessed an impressive progress in the theoretical understanding of transport properties of clean, one-dimensional quantum lattice systems. Many physically relevant models in one dimension are Bethe-ansatz integrable, including the anisotropic spin-1/2 Heisenberg (also called spin-1/2 XXZ chain) and the Fermi-Hubbard model. Nevertheless, practical computations of, for instance, correlation functions and transport coefficients pose hard problems from both the conceptual and technical point of view. Only due to recent progress in the theory of integrable systems on the one hand and due to the development of numerical methods on the other hand has it become possible to compute their finite temperature and nonequilibrium transport properties quantitatively. Most importantly, due to the discovery of a novel class of quasilocal conserved quantities, there is now a qualitative understanding of the origin of ballistic finite-temperature transport, and even diffusive or super-diffusive subleading corrections, in integrable lattice models. We shall review the current understanding of transport in one-dimensional lattice models, in particular, in the paradigmatic example of the spin-1/2 XXZ and Fermi-Hubbard models, and we elaborate on state-of-the-art theoretical methods, including both analytical and computational approaches. Among other novel techniques, we discuss matrix-product-states based simulation methods, dynamical typicality, and, in particular, generalized hydrodynamics. We will discuss the close and fruitful connection between theoretical models and recent experiments, with examples from both the realm of quantum magnets and ultracold quantum gases in optical lattices.

==> integrability_bruno.tex <==
\section{Exploiting integrability}
\label{sec:mazur}


In this section, we will see how integrability affects the finite-temperature transport properties. 
We will stress the important role played by \emph{local} and \emph{quasilocal} conservation laws, showing that they can lead to \emph{ballistic} transport. Specifically, in Sec.~\ref{sec:charges}, we will show that a systematic construction of quasilocal charges provides lower bounds for Drude weights and diffusion constants. In Secs.~\ref{sec:betheansatz} and \ref{sec:GHD}, we will  describe methods to obtain closed-form analytical predictions for these quantities. In particular, Sec.~\ref{sec:DrudeTBA} reports on the predictions for 
spin and energy Drude weights obtained using the Thermodynamic Bethe Ansatz (TBA) formalism, whereas Sec.~\ref{sec:GHD} gives an introduction to GHD and describes its predictions for the Drude weights and diffusion constants of \emph{all} conserved charges. Most of the ideas will be exemplified in the paradigmatic case of the spin-1/2 XXZ chain.

We remark that Secs.~\ref{subsec:BA} and \ref{sec:tba} give a rather detailed introduction to Bethe ansatz and TBA and serve to establish a coherent formalism to express both the TBA results for  transport coefficients and GHD. The reader not interested in technical aspects should skip these subsections and go directly to Secs.~\ref{sec:DrudeTBA} and \ref{sec:GHD}.  

  
  


\subsection{Role of local and quasilocal conserved charges}
\label{sec:charges}

Quantum integrability is based on the existence of two key objects \cite{korepinbook,faddeevreview}. The first one is the $R$-matrix, which can be understood as an abstract unitary scattering operator $\check{R}_{j,l}(\lambda)$ acting over a pair of local finite-dimensional physical Hilbert spaces, ${\cal H}_{j}\simeq {\cal H}_l \simeq \CC^d$. The $R$-matrix depends on a free (complex) spectral parameter $\lambda$ and satisfies the celebrated Yang-Baxter equation. The second key object is the Lax operator $L_{j,a}(\lambda)$, which acts on a pair of Hilbert spaces that are in principle different: the local Hilbert space ${\cal H}_j$ and the so-called ``auxiliary" space $V_a$ of dimension $N_a$, which can be finite or infinite.
These two spaces carry the  physical and auxiliary representation of the quantum symmetry of the problem, respectively. These are most concisely expressed via the so-called RLL relation,\footnote{RLL stands for $R$-matrix -- Lax Matrix -- Lax Matrix} 
\begin{eqnarray}
&\check{R}_{j,l}(\mu) L_{j,a}(\lambda+\frac{\mu}{2})L_{l,a}(\lambda-\frac{\mu}{2}) \nonumber \\
&\;\;\quad\qquad = L_{j,a}(\lambda-\frac{\mu}{2})L_{l,a}(\lambda+\frac{\mu}{2}) \check{R}_{j,l}(\mu). \label{RLL}
\end{eqnarray}
The RLL equation is  another form of the Yang-Baxter relation,
The two-site local Hermitian operator
\begin{equation}
h_{j,j+1}=\frac{{\rm d}\,\,}{{\rm d}\lambda}\check{R}_{j,j+1}(\lambda)\big |_{\lambda=0}
\end{equation} 
then gives the  density of the Hamiltonian
$H=\sum_{j=1}^{L} h_{j,j+1}$ of the corresponding integrable model, where periodic boundary conditions can be assumed for simplicity.

A critical consequence of integrability is the existence of an extensive number of local conserved quantities, which are generated via
logarithmic derivatives 
\begin{equation}
\CCharge = \frac{{\rm d}^n\,\,\,}{{\rm d}\lambda^n} \log \tau(\lambda)\big |_{\lambda=\lambda_0}
\label{LocalCharges}
\end{equation}
of the ``fundamental transfer matrix", an operator over $\bigotimes_j \!\mathcal H_j \simeq (\CC^d)^{\otimes L}$ defined as follows
\begin{equation}
\tau(\lambda) = {\rm tr}_0 L_{1,0}(\lambda) L_{2,0}(\lambda)\cdots L_{L,0}(\lambda). 
\label{fundT}
\end{equation}
Here, $L_{j,0}(\lambda)$ is the Lax operator in the fundamental representation, where the auxiliary space is isomorphic to the local physical space. At the special point $\lambda=\lambda_0$, the Lax operator $L_{j,0}(\lambda)$ degenerates to a permutation operator $L_{j,0}(\lambda_0) = P_{j,0}$, acting as $P \ket{\psi}\otimes \ket{\phi} = \ket{\phi}\otimes\ket{\psi}$. This property is instrumental for showing that $\CCharge=\sum_{l=1}^L \dens_l$ are in fact extensive sums of local densities $\dens_l$. The conservation law property $[H,\tau(\lambda)]\equiv [H,Q_k]\equiv 0$ is then a simple consequence of the RLL relation Eq.~(\ref{RLL}), and similarly, the involution property $[\tau(\lambda),\tau(\mu)]\equiv [Q_j,Q_k]\equiv 0$. In fact, one can fix normalization such that $H=Q_1$.

This construction applies, for example, to the paradigmatic example of the spin-1/2 XXZ chain. In this case, the local Hilbert space is ${\cal H}_j = {\mathbb C}^2$ and $\check{R}_{j,l}(\lambda)$ is the standard 6-vertex $R$-matrix \cite{baxter}. Using the parametrization 
\be
\label{eq:standardparametrisationDelta}
\Delta=\cos(\eta),
\ee
the general Lax operator reads as 
\begin{eqnarray}
\label{eq:Lmatrix}
L_{j,a}(\lambda,s) &=& \frac{2\sin\eta}{\sin\lambda}\left(S_a^+ s^-_j + S_a^- s^+_j\right) \nonumber\\ 
&+&  \cos(\eta S_a^z) \one + 2(\cot\lambda)\sin(\eta S_a^z)s^z_j,  \label{Lax}
\end{eqnarray}
where the local spin operators $s^\alpha_j=(1/2)\sigma^\alpha_j$, $\alpha\in\{+,-,z\}$, act over the local physical space while $S_a^{+,-,z}$ span an irreducible highest-weight representation of the $q$-deformed angular momentum algebra ($q=e^{i \eta}$). This representation depends on a free (complex) parameter
$s\in\CC$ and is generically infinite-dimensional 
\begin{equation}
\begin{split}
S_a^{z} &= \sum_{n=0}^{\infty} (s-n)\ket{n}\bra{n}, \\
S_a^{+} &= \sum_{n=1}^{\infty} \frac{\sin n \eta}{\sin\eta}\ket{n-1}\bra{n},\\
S_a^{-} &= \sum_{n=1}^{\infty} \frac{\sin  (2s-n+1)\eta}{\sin\eta}\ket{n}\bra{n-1}.
\end{split}
\label{s_representation}
\end{equation}
However, either (i) for half-integer spin $s\in \frac{1}{2}\ZZ$ or (ii) for any $s\in\CC$ but root-of-unity anisotropies $\eta = \pi \ell/m$ ($\ell,m$ coprime integers) the above irrep truncates to a finite dimension: $N_a=2s+1$ or $N_a=m$, respectively. In this case, the sums above run up to $n=N_a-1$. One can thus define a general family of commuting transfer matrices
\begin{equation}
\tau(\lambda,s) = {\rm tr}_a L_{1,a}(\lambda,s) L_{2,a}(\lambda,s)\cdots L_{L,a}(\lambda,s),
\end{equation}
satisfying $[H,\tau(\lambda,s)]=0$ for all $\lambda,s$. 

It can be argued that the sequence of local charges $Q_n$ stemming from the fundamental transfer matrix Eq.~(\ref{fundT}) is therefore ``not complete". Consequently, this set  is not sufficient to describe the statistical mechanics of integrable models. Indeed, for unitary irreps with half integer $s$, one can define additional ``quasilocal" charges as 
\begin{equation}
\CCharges = \frac{{\rm d}^n\,\,\,}{{\rm d}\lambda^n} \log \tau(\lambda,s)\big |_{\lambda=\eta/2}\,.
\label{eq:higherconservations}
\end{equation}
For $s>1/2$, these charges are linearly independent from the family of local charges $\CCharges \equiv Q_{n,1/2}$ \cite{Ilievski15a} and are ``essentially local''. 
More formally, for any size $L$, a generic charge $Q=\CCharges$ in the family \eqref{eq:higherconservations} can be written as an extensive series $Q=\sum_r \sum_{l=1}^L {q_{l,r}}$
of $r$-site local densities $q_{l,r}$ with exponentially decaying vector norm  (i.e., 
$\ave{[q_{l,r}]^2} < C e^{-r/\xi}$ for some fixed $C,\xi > 0$). This property, called quasilocality, implies extensivity in the sense
$0 < \lim_{L\to\infty} \ave{Q^2}/L < \infty$. 
Note that Eq.~(\ref{eq:higherconservations}) provides a full set of charges for $|\Delta| \geq 1$, while for $|\Delta| < 1$ one can provide a full classification using the so-called string-charge duality \cite{ilievski2016string}.

All the charges $\CCharges$ generated by unitary representations are {\em even} under a generic $\ZZ_2$ `particle-hole' symmetry of the model, e.g., in the case of the spin-1/2 XXZ chain, under the spin-reversal (spin-flip) transformation $F=\prod_{l=1}^L \sigma^x_l$,
$F \CCharges = \CCharges F$. However, the spin current ${\cal J}^{({\rm S})}$ is odd, ${\cal J}^{({\rm S})} F = -F {\cal J}^{({\rm S})}$,  and hence $
\ave{{\cal J}^{({\rm S})}\CCharges} = 0$. In other words, irrespective of the temperature, these charges cannot contribute to the Mazur bound Eq.~(\ref{eq:MazurD}) at vanishing magnetization.

Nevertheless, one can explore non-unitary representations of the symmetry algebra to search for charges that are not invariant under spin-reversal using the general relation $F \tau(\lambda,s) F^{-1} = \tau(\pi-\lambda,s)^{\rm T}$. For root-of-unity anisotropies $\eta=\pi \ell/m$  ($\ell,m$ coprime integers), this procedure leads to an additional family of quasilocal conserved charges that are non-Hermitian and odd under spin reversal \cite{Prosen2014}. They can be expressed as 
\begin{equation}
\!\! Z(\lambda) =  \frac{\sin{(\lambda})^{2}}{2\eta\sin{(\eta)}}\,\partial_{s} \tau(\lambda,s)\vert_{s=0}-
\frac{\sin{(\lambda)}\cos{(\lambda)}}{\sin{(\eta)}}\, \Mtot\!,
\label{eqn:Zdef0}
\end{equation}
where $\lambda$ lies inside the 
analyticity strip ${\cal S}=\{ \lambda\in\CC; |{\rm Re}\,\lambda - 
\frac{\pi}{2}| < \frac{\pi}{2m}\}$ and  $\Mtot=\sum_{r=1}^L \sz{r}$ denotes the 
total magnetization in the $z$ direction. 

\subsubsection{Lower bound on spin Drude weight at high temperature}
\label{sec:lowerbounddrude}

Since the quasilocal charges generated from non-unitary representations are not spin-reversal invariant, they have a non-vanishing overlap with the spin current and may contribute to the Mazur bound. 
For example, in the high-temperature regime ($\beta\to 0$), the overlap is also extensive, $\ave{ Z(\lambda) {\cal J}^{({\rm S})}} = i L/4$, yielding a finite
contribution to Eq.~(\ref{eq:MazurD}). However, the $Z(\lambda)$ are not mutually orthogonal and  their overlaps are given by the following analytic kernel
\begin{eqnarray*}
K(\lambda,\mu) &=& \lim_{L\to\infty}\frac{\ave{Z(\bar{\lambda})^\dagger Z(\mu)}}{L} \nonumber \\
&=& -\frac{\sin{(\lambda)}\sin{(\mu)}\,\sin((m-1)(\lambda+\mu))}{2\sin^2{(\eta)}\sin{(m(\lambda+\mu))}}
 \end{eqnarray*}
 while
 ${\ave{Z(\lambda)Z(\mu)} \equiv 0}$. The Mazur bound for the spin-Drude weight generally follows \cite{Ilievski2013} from finding an extremum of  the nonnegative action
 \begin{equation}
 {\cal S}[f]:= \lim_{t\to\infty}\lim_{L\to\infty} \frac{1}{L} \ave{(B_{L,t}[f])^\dagger B_{L,t}[f]} \ge 0,
 \end{equation} 
  with respect to an unknown function $f(\lambda)$. Here, we introduced 
 \begin{equation}
 B_{L,t}[f(\lambda)] := \frac{1}{t}\int_0^t {\rm d} s\, {\cal J}^{(S)}(s) - \int_{{\cal S}} {\rm d}^2\lambda\, f(\lambda)Z(\lambda).
 \end{equation} 
The variation $\delta S/\delta f(\lambda)=0$ results in the Fredholm equation of the first kind on a two-dimensional (complex) domain ${\cal S}$
 \begin{equation}
 \int_{\cal S} d^2 \mu K(\lambda,\mu)f(\mu) = \ave{Z(\lambda)j^{({\rm S})}}\,, 
\end{equation}
 which for the spin-1/2 XXZ chain with $\Delta=\cos(\pi \ell/m)$ yields 
 \begin{equation}
 f(\lambda) = \frac{m \sin^2(\pi/m)}{i \pi |\sin\lambda|^4}.
 \end{equation} 
 This in turn results in the following rigorous lower bound for the leading coefficient of the Drude weight ${\tilde {\cal D}^{(S)}_{\rm w}}$ in the high-temperature expansion
 \begin{eqnarray} \label{eq:prosen_bound}
{\tilde {\cal D}^{\rm (S)}_{\rm w}} &=& \lim_{\beta\to 0} \frac{\Dws}{\beta} \ge \frac{1}{2}\int_{\cal S} d\lambda^2 f(\lambda)\ave{Z(\lambda)j_0^{({\rm S})}} \nonumber \\
&=& \frac{1}{16} \frac{\sin^{2}{(\pi \ell/m)}}{\sin^{2}{(\pi/m)}}
\left(1 - \frac{m}{2\pi}\sin{\left(\frac{2\pi}{m}\right)}\right).
 \end{eqnarray}
Note that the r.h.s. of~\eqref{eq:prosen_bound} is a nowhere continuous function of $\Delta$ whose graph is a fractal set.
The dependence on $\Delta$ is illustrated in Fig.~\ref{fig:prosen_bound}.
 
We refer the reader to  Sec.~\ref{sec:xxz} for a detailed discussion of the saturation of this bound 
and \cite{Matsui2020} for explaining why the natural non-quasilocal extension of the quasilocal charges given in Eq.~\eqref{eq:higherconservations}  cannot improve the bound. 
A more comprehensive review on quasilocal charges can be found in \cite{Ilievski2016}, whereas the extension of Drude weights and quasilocal charges to integrable periodically driven (Floquet) systems is given in \cite{Ljubotina2019a}.

\begin{figure}[t]
\begin{center}
%\includegraphics[width=0.90\linewidth]{figs_xxz/xxz_bound}
\includegraphics[width=0.90\linewidth]{xxz_bound}
\caption{(Color online) Lower bound for the spin Drude weight $\Dws$ of the spin-1/2 XXZ chain according
to Eq.\ (\ref{eq:prosen_bound}), as obtained in \cite{Prosen2013}, and
another lower bound for $\Dws$, as obtained earlier in \cite{Prosen2011}.
Both bounds exhibit a pronounced fractal-like (i.e., nowhere continuous)
dependence on the anisotropy parameter $\Delta$.}
\label{fig:prosen_bound}
\end{center}
\end{figure}

 \subsubsection{Lower bounds on spin diffusion constant at high temperature}
\label{sec:lowerbound_diff}

In typical integrable models, e.g., the spin-1/2  XXZ chain for $|\Delta| \ge 1$ 
or the 1d Fermi-Hubbard model, the spin or charge Drude weight vanishes at zero 
magnetization $\magdens= 2 \langle \Mtot\rangle/L=0$  
or in the half-filled sector $\rho = N/L=1/2$, respectively. However, moving slightly away from half filling, one typically obtains a finite Drude weight. More precisely, calling $\delta$ the small deviation from either zero magnetization or half filling, one observes a Drude-weight scaling as $\Dw^{(Q)} \propto \delta^2$. At first sight, this seems to exclude the onset of spin diffusion: a finite Drude weight implies a diverging diffusion constant. Nevertheless, for large $L$, the Hilbert-space sector at $\delta=0$ dominates over all sectors with $\delta\ne 0$. Therefore, one may argue that, after performing a careful (grand)canonical average, the two effects compensate each other giving rise to a finite spin- or charge-diffusion constant in the thermodynamic limit.

In fact, this argument can be  justified rigorously by studying the Mazur bound for the dynamical susceptibility in a double-scaling limit, $L\to \infty$ and $t \to \infty$ with $L/t > v_{\rm LR}$, giving rise to a universal lower bound on the 
diffusion constant $D^{(Q)}$ in terms of the curvature of the Drude weight ${\cal D}^{(Q)}_{\rm w}(\beta,\delta)$ around $\delta=0$: \cite{Medenjak2017} [see also \cite{Spohn2018}].
For spin transport, one obtains: 
\begin{equation}
	\DS(\beta)\geq \frac{1}{8\beta v_{\rm LR}\chi(\beta) f_1(\beta)} \frac{\partial^2}{\partial \delta^2}\Dws(\beta,\delta)\Bigr|_{\delta=0},
	\label{diflb}
\end{equation}
where $ v_{\rm LR} $ is the Lieb-Robinson velocity \cite{liebrobinson}, and 
\be
f_1(\beta)=\lim_{L\to\infty}\frac{1}{2L} \frac{\partial^2}{\partial \delta^2} F_{L}(\beta,\delta)|_{\delta=0}
\ee
is a second derivative of the free-energy density 
at zero magnetization, while $\chi(\beta)$ is the static susceptibility 
         $
	{\chi(\beta)}/{\beta}=\lim_{L\to\infty}{\langle (\Mtot)^2 
\rangle-(\langle \Mtot \rangle)^2}/L
	$.
The inequality holds in general, even for a nonintegrable system, if there exist conserved quantities which would make Drude weights nonvanishing away from the symmetric Hilbert-space sector $\delta=0$. However, for integrable systems with a well-understood quasiparticle content, such as the spin-1/2 XXZ chain, the inequality can be further refined by decomposing the contribution to the diffusion constant in terms of the curvatures of the Drude weight contributions
associated to independent Bethe-ansatz quasiparticle species (see Sec.~\ref{sec:GHDDrude}). In this case, the velocity $v_{\rm LR}$ can be replaced by the corresponding dressed quasiparticle  velocity \cite{Ilievski2018}.

One can approach lower bounds on diffusion constants from another angle. In the same way as for the Mazur bound, Eq.~(\ref{eq:MazurD}) suggests that a non-vanishing high-temperature Drude weight is connected to the existence of linearly extensive --- i.e., proportional to the volume --- (quasi)local charges. One might therefore argue that a non-vanishing high-temperature diffusion constant suggests the existence of 
conserved charges which are quadratically extensive. 
Indeed, for any locally interacting lattice system, the existence of an almost conserved operator $Q$ (where $[H,Q]={\rm boundary\; terms}$), satisfying 
$0 < q:=\lim_{L\to\infty} \langle Q^2 \rangle/L^2 <\infty$ and $Q^j:=\lim_{L\to\infty}\langle j_r^{(Q')}  Q\rangle$ finite, which has has an overlap with any one current operator $j_r^{(Q')}$), leads to a rigorous bound on high-temperature diffusion constants \cite{TP2014QuadCharges}
associated with that current 
\be
\D^{(Q')}(\beta\to 0) \ge \frac{ |Q^j|^2} {8 v_{\rm LR} q}.
\ee
This gives, e.g., nontrivial lower bounds for spin-diffusion constants in the spin-1/2 Heisenberg chain as well as for  spin- and charge-diffusion constants for the  1d Fermi-Hubbard model. The bound has been recently generalized and formalized within the method of ``hydrodynamic projections" in \cite{Doyon2019QuadCharges} (cf.\ Sec.~\ref{sec:GHDDrude}), where similar ideas were also used to provide bounds on anomalous (e.g., superdiffusive) transport, i.e., to estimate the dynamical exponents.

\subsection{Bethe Ansatz}
\label{sec:betheansatz}

Here, we consider an important subclass of integrable models: those treatable by the collection of techniques grouped under the name of Bethe ansatz. The key property of these models is that their energy eigenstates can be expressed as scattering states of stable quasiparticles~\cite{korepinbook, faddeevreview, esslerbook}. This gives direct access to their energy spectrum and, more generally, to their thermodynamic properties. Although the stable quasiparticles of integrable models generically undergo nontrivial scattering processes, integrability ensures that every scattering process can always be decomposed into a sequence of two-particle scatterings.

Focussing on the paradigmatic example of the spin-1/2 XXZ chain, we will 
introduce the central equations of Bethe ansatz --- the Bethe equations --- 
which give access to all possible eigenstates of the systems. Then, we will 
explain how to take their thermodynamic limit, arriving at the so called 
thermodynamic Bethe ansatz (TBA) description~\cite{Takahashi:1999aa}, where one 
characterizes the eigenstates in terms of ``densities" of quasiparticles. 
Finally, we will recall some results for the energy and spin Drude weight 
obtained using TBA.    

\subsubsection{Bethe Equations via Algebraic Bethe Ansatz}
\label{subsec:BA}

There are two known routes to derive the Bethe equations. The first one consists in writing an ansatz many-body wave-function in real (coordinate) space. This is the original method introduced in \cite{Bethe} and is now known as coordinate Bethe ansatz. The second, more recent route consists of constructing a basis of eigenstates of the fundamental transfer matrix \eqref{fundT} for all values of the spectral parameter $\lambda$ (cf. Sec.~\ref{sec:charges}). This is always possible since transfer matrices with different spectral parameters commute. Since the Hamiltonian is proportional to the logarithmic derivative of the transfer matrix, these states are also eigenstates of $H$. This second route, called algebraic Bethe ansatz, is more powerful: it gives direct insights into the conservation laws of the system and correlation functions~\cite{korepinbook, faddeevreview, esslerbook}. Here, we follow the latter approach. 

The starting point is to consider the ($s=1/2$) ``monodromy matrix" defined as 
\be
\!\!\!\!\!M_{a}(\lambda,\tfrac{1}{2})\! =\! L_{1,a}(\lambda) L_{2,a}(\lambda)\!\cdots\! L_{L,a}(\lambda) \!\!=\!\!
\begin{bmatrix}
A(\lambda) & B(\lambda)\\
C(\lambda)& D(\lambda)
\end{bmatrix}\!\!.
\label{fundM}
\ee
This is a matrix in the auxiliary space $V_a \simeq \CC^2$ whose elements are operators in $\mathcal \bigotimes_j \mathcal H_j \simeq (\CC^d)^{\otimes L}$ and its trace over the auxiliary space gives the transfer matrix for ${s=1/2}$, i.e., ${{\rm tr}_a M_{a}(\lambda,\tfrac{1}{2})=A(\lambda)+D(\lambda)=\tau(\lambda,\tfrac{1}{2})}$. In particular, for the spin-1/2 XXZ chain, $\tau(\lambda,\tfrac{1}{2})$ coincides with the fundamental transfer matrix $\tau(\lambda)$ ($V_a\simeq \mathcal H_j \simeq \CC^2$). This    is exactly the object that we want to diagonalize. Although this treatment can be extended also to systems with larger local Hilbert spaces with dimensions  $d>2$, from now on, we stick to this simple case and diagonalize $\tau(\lambda)=\tau(\lambda,\tfrac{1}{2})$. We also drop the label $\tfrac{1}{2}$ since we will always deal with objects in the fundamental representation.

The algebraic Bethe ansatz procedure follows closely the diagonalization of a one-particle harmonic oscillator via creation and annihilation operators, and can be ideally divided into two steps~\cite{korepinbook, faddeevreview, esslerbook}. First, one determines the algebra obeyed by the operators $A(\lambda), \ldots, D(\lambda)$, then one finds a ``highest weight'' state from which to construct an irreducible representation: the vector space where the irreducible representation acts plays the role of a Hilbert space of the system. The first step is conveniently accomplished using Eq.~\eqref{RLL}, from which we find the ``fundamental" commutation relations of the monodromy matrix (equivalent to Eq.~\eqref{RLL} for $V_a\simeq \mathcal H_j$)
\begin{align}
\check{R}_{a,b}(\mu)& M_{a}\left(\lambda+\frac{\mu}{2}\right)M_{b}\left(\lambda-\frac{\mu}{2}\right) \notag\\
&= M_{a}\left(\lambda-\frac{\mu}{2}\right)M_{b}\left(\lambda+\frac{\mu}{2}\right)\check{R}_{a,b}(\mu)\,.
\label{eq:RMM}
\end{align}
Here, $a$ and $b$ label two different auxiliary spaces $V_a$ and $V_b$, with $V_a\simeq V_b \simeq \CC^2$. Using the standard 6-vertex $R$-matrix \cite{baxter}, we select the following components of Eq.~\eqref{eq:RMM} 
\begin{align}
&\!\!\![B(\lambda), B(\mu)]=0 \label{eq:Alg1}\\
&\!\!\!A(\lambda)B(\mu) \!\!=\!\! f(\lambda-\mu)B(\mu) A(\lambda) \!+\!g(\lambda-\mu) B(\lambda) A(\mu),\label{eq:Alg2}\\
&\!\!\!A(\lambda)D(\mu) \!\!=\!\! f(\mu-\lambda)D(\mu) A(\lambda) \!+\!g(\mu-\lambda) B(\lambda) A(\mu),\label{eq:Alg3}
\end{align}
where ${f(\lambda)=\cos(\lambda-\eta)/\cos\lambda}$ and ${g(\lambda)=\sin\eta/\cos\lambda}$ (we recall that ${\cos\eta=\Delta}$). The second step is achieved by identifying a special state ${\ket{\Omega}\in\bigotimes_{j} \mathcal H_j}$ (the ``pseudovacuum") fulfilling 
\begin{eqnarray}
&&A(\lambda)\ket{\Omega}=a(\lambda)\ket{\Omega},\qquad D(\lambda)\ket{\Omega}=d(\lambda)\ket{\Omega},\\
&& C(\lambda)\ket{\Omega}=0\,,
\label{eq:pseudovacuum}
\end{eqnarray}
where $a(\lambda), d(\lambda)\in\mathbb C$. Note that for the spin-1/2 XXZ chain, the ferromagnetic state $\bigotimes_j \ket{\uparrow}_j\equiv {\ket{\uparrow\ldots\uparrow}}$ can be chosen as a pseudovacuum. Indeed, using the Lax operator \eqref{eq:Lmatrix} for $s=1/2$, we have 
\be
L_{j,a}(\lambda) \ket{\uparrow}= 
\begin{bmatrix}
 k_+(\lambda)\ket{\uparrow} & \ast  \\
 0 &   k_-(\lambda) \ket{\uparrow}\\ 
\end{bmatrix}\,,
\ee
where we introduced ${k_\pm(\lambda)= \sin(\lambda\pm\eta/2)/\sin\lambda}$ and $\ast$ is a state in the local physical space $\mathcal H_j$ which is not relevant for our analysis. Plugging this relation into the definition of the monodromy matrix Eq.~\eqref{fundM}, we find that ${\ket{\uparrow\ldots\uparrow}}$ fulfills \eqref{eq:pseudovacuum} with $a(\lambda)=(k_+(\lambda))^L$ and $d(\lambda)=(k_-(\lambda))^L$. We stress that integrability (i.e., the existence of an $R$ matrix and a Lax operator fulfilling Eq.~\eqref{RLL}) does not generically imply the existence of a pseudovacuum (although this happens in many relevant models~\cite{korepinbook}). This is the ultimate reason why not all integrable models are Bethe-ansatz solvable.  

Given a pseudovacuum $\ket{\Omega}$ and the commutation relations Eqs.~\eqref{eq:Alg1}--\eqref{eq:Alg3}, we find that all states of the form 
\be
\ket{\Psi_{\boldsymbol \lambda}} = \prod_{j=1}^N B(i\lambda_j+\tfrac{\pi}{2})\ket{\Omega},\qquad N\leq L,
\label{eq:Bethestate}
\ee
are eigenstates of $\tau(\lambda)$ provided that the set of rapidities $\boldsymbol \lambda=\{\lambda_j\}$ fulfills 
\be
\!\!\!\left[\frac{\sinh(\lambda_j+i\eta/2)}{\sinh(\lambda_j-i\eta/2)}\right]^L \!\!= -\prod_{k= 1}^N \left[\frac{\sinh(\lambda_j-\lambda_k+i\eta)}{\sinh(\lambda_j-\lambda_k-i\eta)}\right],
\label{eq:BetheEquations}
\ee
for $j=1,\ldots,N$. These are the illustrious Bethe equations, first found in \cite{Bethe} for $\Delta=1$ and then in \cite{Orbach} for generic $\Delta$. In our framework, they originate when requiring that after commuting $\tau(\lambda)$ with $B(\lambda)$, the state \eqref{eq:Bethestate} remains of the same form, i.e., contributions arising from the second terms on the r.h.s. of Eqs.~\eqref{eq:Alg2} and \eqref{eq:Alg3} (the ``unwanted contributions") vanish. All Bethe-ansatz integrable models produce sets of nonlinear, coupled, algebraic equations of this form. In some cases, however, one needs to repeat the procedure multiple times before finding the eigenstates of the Hamiltonian. This produces multiple sets of equations similar to Eq.~\eqref{eq:BetheEquations}, involving different sets of rapidities, which are coupled together. This procedure is known as nested Bethe ansatz and is necessary, e.g., for the Fermi-Hubbard model. For simplicity, we restrict the discussion  to the non-nested case in our presentation. 

Instead of reporting the eigenvalue of $\tau(\lambda)$ in the state \eqref{eq:Bethestate} (see, e.g., \cite{korepinbook, faddeevreview} for the explicit form), here, we consider those of local conserved charges. 
The eigenvalues of quasimomentum\footnote{On the chain, the quasimomentum operator is defined as $-i\log \tau(\lambda_0)$ ($\tau(\lambda_0)$ acts as the one-site-shift operator.} and the Hamiltonian read as 
\be
\!\!P \!=\!\! \left[\sum_{k=1}^{N} p(\lambda_k, \tfrac{1}{2})\!\right]\!{\rm mod} 2\pi,\qquad E\!=\!\!\sum_{k=1}^{N} e(\lambda_k)+e_0 L,
\label{eq:EVEP}
\ee
where we set ${p(\lambda, s)\!\!=\!i\log\left[{\sinh(\lambda-i\eta s)}/\sinh(\lambda+i\eta s)\right]}$, ${e(\lambda)=\!-\sin\eta/2\, \partial_\lambda p(\lambda, \tfrac{1}{2})}$ and ${e_0={\Delta}/{4}}$. An expression similar to the one for the energy holds for higher local (and quasilocal) conservation laws \eqref{eq:higherconservations}. In particular, in the eigenvalue of $\CCharges$ the function $e(\lambda)$ is replaced by ${q_n(\lambda,s)=(-\sin\eta/2)^n \partial_\lambda^n p(\lambda, s)}$ while the constant shift $e_0$ is replaced by 0.  

The Bethe equations might be viewed as convoluted quantization conditions for the momenta (or better the ``rapidities'') of a gas of quasiparticles confined in a finite volume $L$. However, one should be careful  with such an interpretation as the solutions to these equations are generically \emph{complex}: this is a common feature of many Bethe-ansatz integrable models. 


To understand the distribution of the roots in the complex plane, it is useful to look at the solutions for $L\to\infty$ and fixed $N$~\cite{Takahashi:1999aa, esslerbook}. In this case, any ${\rm Im}[\lambda_j]\neq0$ causes the l.h.s. to either go to infinity or to 0. Requiring the r.h.s. to do the same forces the solutions to follow ordered patterns in the complex plane known as ``strings". 
%
Strings can be interpreted as stable bound states formed by the elementary particles \cite{esslerbook} and appear in all Bethe-ansatz integrable models with complex rapidities, but their specific form depends on the model and on the values of its parameters. 
%
Specifically, in the spin-1/2 XXZ chain, the string-structure depends on whether $\eta$ is real ($|\Delta|<1$) or imaginary ($|\Delta|>1$). For instance, for $\eta\in\mathbb R$, we have strings of the form~\cite{Takahashi:1999aa} 
\be
\lambda_{\alpha, a}^k = \lambda_\alpha^k+i\frac{\eta}{2}(n_k+1-2a)+i \frac{\pi}{4}(1-\upsilon_k)+\delta_{\alpha,a}^k,
\label{eq:strings}
\ee
where $\lambda_\alpha^k\in\mathbb R$ is called ``string center", $k=1,\ldots,N_s$ is called ``string type", $\alpha=1,\ldots,M_k$ labels different strings of the same type, and $a=1,\ldots,n_k$ labels rapidities in the same string. Finally, the ``string deviations" $\delta_{\alpha,a}^k$ are exponentially small in $L$. 

The number $N_s$ of type of strings, the ``length" $n_k$ of the $k$-th string, and its ``parity" $\upsilon_k$ depend on $\eta$ in a discontinuous way: they change drastically depending on whether $\eta/\pi$ is rational. For example, for $\eta=\pi/m$, we have $N_s=m$, ${n_k=(k-1)(1-\delta_{k,m})+1}$, and $\upsilon_k=1-2\delta_{k,m}$. A similar parameterisation of strings can be performed also for $i\eta\in\mathbb R$ and more generally, for other Bethe-ansatz integrable models~\cite{Takahashi:1999aa}.  

\subsubsection{Thermodynamic Bethe Ansatz}
\label{sec:tba}

For small numbers $N$ of rapidities, the Bethe equations can be easily solved on a computer [see, e.g., \cite{hagemansthesis, Shevchukthesis}]. For a full classification of the solutions of Eq.~\eqref{eq:BetheEquations}, this is feasible for  for $N\leq L=10$.  However, this provedure becomes quickly impractical when $N$ and $L$ increase. In particular, to study the thermodynamic limit --- $N,L\to\infty$ with finite $N/L$ --- a brute force numerical solution of the equations is unfeasible and some analytical treatment becomes unavoidable. The standard approach --- known as thermodynamic Bethe ansatz (TBA) --- is based on the crucial assumption that the solutions to Eq.~\eqref{eq:BetheEquations} continue to follow the string patterns \emph{even at finite density} \cite{Bethe,Taka1971}, i.e., when $N$ is not fixed but goes to infinity with $L$. Although this assumption --- usually called \emph{string hypothesis} --- does not strictly hold for all states in large but finite systems, it is believed to describe exactly the thermodynamic properties of all Bethe-ansatz integrable models. In particular, the string hypothesis has been proven to be self-consistent for the spin-1/2 XXZ chain at finite temperature \cite{Tsvelik83}. A more rigorous alternative to the string hypothesis exists \cite{Kluemper92,Kluemper93,SuzukiInoue87} and is often referred to as quantum transfer-matrix approach. 
Even though this approach is very powerful, it is generically less versatile than TBA (currently most of the results have been found for thermal states). Importantly, the two approaches have been proven to give an equivalent description of the thermodynamic properties of the spin-1/2 XXZ chain at finite temperatures \cite{Kluemper92, Kuniba1998}. 

Embracing the string hypothesis and multiplying together all Bethe equations referring to particles in the same string one arrives at a set of equations --- known as Bethe-Takahashi equations --- for the real string centers [cf.~Eq.~\eqref{eq:strings}]. These equations can readily be viewed as quantization conditions for the momenta of the original particles and all their bound states and are most commonly expressed in ``logarithmic form" (taking $-i\log[\cdot]$ of both sides). In particular, the Bethe-Takahashi equations for the spin-1/2 XXZ chain read as \cite{Takahashi:1999aa} 
\be
L \theta_j(\lambda_\alpha^j)-
{\sum_{k=1}^{N_s}\sum_{\gamma=1}^{M_k}}\Theta_{jk}(\lambda_\alpha^j-\lambda_\gamma^k)=2\pi I_{\alpha}^{(j)}\,,
\label{eq:BetheTaka}
\ee  
where the ``quantum numbers" $I_{\alpha}^{(j)}$ are integer (half-odd integers) for odd (even) $L-M_j$ (also their allowed ranges depend on $\{M_j\}$) and the string centres $\lambda_\alpha^j$ lie in the symmetric interval $[-\Lambda,\Lambda]\subset \mathbb R$ while the smooth functions $\theta_j(x)$ and $\Theta_{ij}(x)$ can be expressed as 
\begin{align}
\theta_j(x)=&f(x;n_j,\upsilon_j),\\ 
\Theta_{ij}(x)=&f(x;|n_i-n_j|,\upsilon_i\upsilon_j)+f(x;n_i+n_j,\upsilon_i\upsilon_j)\notag\\
&+2 \!\!\!\!\!\!\!\!\!\!\! \sum_{k=1}^{\min(n_i,n_j)-1} \!\!\!\!\!\!\!\!\!\!\!f(x;|n_i-n_j|+2k,\upsilon_i\upsilon_j).
\end{align}
Both $\Lambda$ and the form of the auxiliary function $f(x; n; \upsilon)$ depend on whether  $|\Delta|<1$ or  $|\Delta|\geq1$; their form is reported in Table~\ref{table:XXZ}. 


\begin{table}
\begin{tabular}{|c|c|c|}
 \hline
 & $|\Delta|<1$ &  $|\Delta|\geq1$  \\
 \hline
$\Lambda$ & $\infty$ & $\pi/2$ \\
\hline
$\frac{f(x; n; \upsilon)}{2}$ & $
\begin{cases}
\upsilon\,{\rm atan}\!\!\left[\frac{\tanh x}{[\tan\frac{n \gamma}{2}]^{\upsilon}}\right] &n\gamma\notin\mathbb Z\\
0 &n\gamma\in\mathbb Z\\
\end{cases}$ &${\rm atan}\!\!\left[\frac{\tan x}{\tanh\frac{n \gamma}{2}}\right]\!\!+\!\pi \lfloor \frac{x}{\pi}+\frac{1}{2}\rfloor$ \\[1.5pt]
   \hline
\end{tabular}
\caption{Auxiliary function $f(x; n; \upsilon)$ for the spin-1/2 XXZ chain for $\Delta=\cos\eta$. We defined $\gamma\equiv|\eta|$. \label{table:XXZ}}
\end{table}

Furthermore, by substituting the string hypothesis in the expectation value of the energy density [see Eq.~\eqref{eq:EVEP}], we have 
\be
E\!=\!\!\sum_{k=1}^{N_s}\sum_{\gamma=1}^{M_k} e_k(\lambda_\gamma^k)+e_0 L,
\label{eq:energySH}
\ee
where the functions ${e_k(\lambda)\!\equiv\! A(\Delta)\partial_\lambda \theta_k(\lambda)}$ with ${A(\Delta)=-{\rm sgn}(\Delta+1) \sqrt{|\Delta^2-1|}/2}$ are known as ``bare energies''. We see that the energy of an eigenstate is obtained by summing up the bare energies of all quasiparticles characterizing it. A similar expression holds for higher conservation laws.  



The set $\{I_{\alpha}^{(j)}\}$ is in one-to-one correspondence with the set of string centres (or ``particle rapidities") $\{\lambda_{\alpha}^{(j)}\}$ and can be used to specify the state of the system, much like momentum occupation numbers in free systems. We note in passing that the correspondence between $\{I_{\alpha}^{(j)}\}$ and the solutions of the Bethe equations has been used to prove the combinatorial completeness of Bethe ansatz for the XXZ chain~\cite{KirillovCompleteness, KirillovCompleteness2} and for the Fermi-Hubbard model \cite{CompletenessHubbbard}. The correspondence is explicitly established by introducing the ``counting functions" 
\be
{z_j(x|\{\lambda_{\alpha}^{(j)}\}) \equiv \theta_j(x)-\frac{1}{L}{\sum_{k=1}^{N_s}\sum_{\gamma=1}^{M_k}}\Theta_{jk}(x-\lambda_\gamma^k)}.
\ee
These functions are monotonic in $x$ and, by definition, satisfy ${z_j(\lambda_{\gamma}^{(k)} |\{\lambda_{\alpha}^{(j)}\})=2\pi I^{(k)}_\gamma /L}$ (this is just a rewriting of \eqref{eq:BetheTaka}). There exist, however, some ``hole rapidities" ${\{\bar \lambda_\gamma^j\}\not\subset\{\lambda_{\alpha}^{(j)}\}}$ such that ${z_j(\bar \lambda_\gamma^j |\{\lambda_{\alpha}^{(j)}\})=2\pi J^{(j)}_\gamma /L}$ with $\{J_{\alpha}^{(j)}\}$ integers (or half-odd integers)  in the allowed range to be quantum numbers but not appearing in $\{I_{\alpha}^{(j)}\}$ (they can be thought of as empty slots).  

In the thermodynamic limit, both particle and hole rapidities become dense in $[-\Lambda,\Lambda]$ (differences of neighboring rapidities scale like $L^{-1}$) and it is convenient to switch  to a ``coarse grained" description of the system in terms of densities of particles $\{\rho_j(\lambda)\}$ and of holes $\{\rho^h_j(\lambda)\}$ ($h$ stands for ``hole"). It is easy to verify that $2 \pi \sigma_j(\rho_j(\lambda) +\rho^{h}_j(\lambda))= \lim_{L\to\infty} \partial_\lambda z_j(\lambda|\{\lambda_{\alpha}^{(j)}\})$, where the sign ${\sigma_j=\{\pm1\}}$ accounts for strings where ${z_j(x|\{\lambda_{\alpha}^{(j)}\})}$ is monotonically decreasing (they occur for ${|\Delta|<1}$) \cite{Takahashi:1999aa}. Computing the derivative explicitly, we find the so called thermodynamic Bethe-Takahashi equations
\be
\rho_j^t(\lambda) \equiv \rho_j(\lambda) +\rho^{h}_j(\lambda)= \sigma_j a_j(\lambda) - \sum_{k=1}^{N_s} \sigma_j T_{jk}\ast \rho_k (\lambda).
\label{eq:TBT}
\ee
Here, we introduced the driving ${a_j(\lambda)=(1/2\pi)\partial_\lambda \theta_j(\lambda)}$, and the kernel ${T_{jk}(\lambda)=(1/2\pi)\partial_\lambda \Theta_{jk}(\lambda)}$ (encoding all information about the interactions), while $\ast$ denotes the convolution $f\ast g(x)=\int_{-\Lambda}^\Lambda {\rm d}y f(x-y)g(y)$.

Equations \eqref{eq:TBT} fix the densities of holes in terms of the densities of particles. In other words, for each state, they provide the densities $\rho_j^t(\lambda)$ of ``rapidity slots" (called ``vacancies")  that can be occupied by a particle. Due to the interactions, the density of slots depends on the state [cf. the second term on the r.h.s.\ of Eq.~\eqref{eq:TBT}]. Integral equations of this form are very common in TBA. In the following, we will find many instances of these equations with the same kernel but different driving functions. 

We remark that,  even though each eigenstate of the Hamiltonian corresponds to a set of densities $\{\rho_j(\lambda)\}$, the correspondence is generically not one-to-one: in a large finite volume $L$, there are approximately $\exp[L s[\rho]]$ eigenstates of the Hamiltonian corresponding to the same set of densities $\{\rho_j(\lambda)\}$. Here, we introduced the Yang-Yang Entropy density ${s[\rho]=\sum_{k} \!\int \!{\rm d}\lambda (\rho^t_k\log\rho^t_k-\rho_k\log\rho_k-\rho^h_k\log\rho^h_k})$. This fact is often referred to by saying that the densities of rapidities specify a ``macrostate" of the system, as opposed to a single eigenstate of the Hamiltonian that is called ``microstate".     


The densities of rapidities in principle allow one to compute the expectation values of all local operators in the thermodynamic limit. In practice, however, explicit expressions are known only for few classes of observables (see also Sec.~\ref{sec:GHD}). A relevant example is that of  local (and quasilocal) conserved-charge densities. Considering the density of the generic charge $Q$, we have 
\begin{align}
q[\rho]&=\sum_{k=1}^{N_s} \!\int \!\!{\rm d}\lambda\, q_k(\lambda)\rho_k(\lambda),
\label{eq:charge}
\end{align}
where the set of functions $q_k(\lambda)$ specifies the charge and it is often called ``bare charge". For example, the energy density is obtained by replacing $q_k(\lambda)$ with $e_k(\lambda)$ and adding the constant shift $e_0$ while setting $q_k(\lambda)=q_{n,k}(s,\lambda)$. For some appropriate $q_{n,k}(s,\lambda)$, one reproduces the density of  higher conservation laws \eqref{eq:higherconservations}. In particular, for the densities $q_n[\rho]$ of the higher local conserved charges \eqref{LocalCharges}, we have $q_{k}(\lambda)=q_{n,k}(\lambda)=(A(\Delta) \partial_\lambda)^{n+1} \theta_k(\lambda)$. 
 

TBA can also be used to analyze excitations over macrostates.  Let us take a large finite volume $L$ and consider the system in one of the microstates corresponding to the densities $\{\rho_j(\lambda)\}$. Injecting an extra string of type $j$ and rapidity $\lambda$ induces a change in the expectation values of the conserved charges
\be
L q[\rho] \mapsto L q[\rho]+ q_j^d(\lambda).
\ee
This $O(L^0)$ quantity is called ``dressed charge" and is related to the bare charge of Eq.~\eqref{eq:charge} by the following integral equation for first derivatives 
\be
\partial_\lambda q^d_j (\lambda)= \partial_\lambda q_j(\lambda) - \sum_{k=1}^{N_s}\sigma_k \left[T_{jk}\ast  \vartheta_k \partial_\lambda q^d_k \right](\lambda).
\label{eq:dressing1}
\ee
where we introduced the ``filling" function 
\be
\vartheta_j(\lambda)\equiv \frac{\rho_j(\lambda)}{\rho^t_j(\lambda)}.
\label{eq:thetafun}
\ee
Even though the momentum is only conserved modulo $2\pi$, a dressed momentum is well defined as long as $p_j^d(\lambda)<2\pi$. In particular, since the bare charge related to the momentum is  $\theta_j(\lambda)$ [cf.\  Eq.~\eqref{eq:EVEP}], the dressed momentum fulfills $ \partial_\lambda p_j^d(\lambda)= 2\pi \sigma_j \rho^t_j(\lambda)$. This can be established comparing the equation for the dressed momentum with Eq.~\eqref{eq:TBT} and allows us to express the group velocity of the excitation $(\lambda,j)$ as 
\be
v^d_{j}(\lambda)=\frac{\partial_\lambda e^d_{j}(\lambda)}{\partial_\lambda p^d_{j}(\lambda)}=\frac{\partial_\lambda e^d_{j}(\lambda)}{2\pi \sigma_j \rho^t_j(\lambda)}\,.
\label{eq:velocityrhot}
\ee
In other words, $2\pi \sigma_j \rho^t_j(\lambda) v^d_{j}(\lambda)$ fulfills Eq.~\eqref{eq:dressing1} with $\partial_\lambda e_{j}(\lambda)$ as a driving. In addition to the dressed charge, we can associate  another ``dressed" quantity, sometimes called the ``effective charge",
to each quasilocal conservation law (and also to the momentum).
For a given bare charge $q_j(\lambda)$, we define the associated effective charge $q_j^{\rm eff}(\lambda)$ as the solution of the following Eq.~\eqref{eq:dressing}, which has $q_j(\lambda)$ as its driving term, 
\be
q^{\rm eff}_j (\lambda)= q_j(\lambda) - \sum_{k=1}^{N_s}\sigma_k \left[T_{jk}\ast  \vartheta_k  q^{\rm eff}_k \right](\lambda).
\label{eq:dressing}
\ee
Note that in this case, one directly ``dresses" the charge and not its derivative and hence dressed and effective charges do not coincide. We have, however, ${\partial_\lambda (q_j^{\rm d}(\lambda))=(\partial_\lambda q_j(\lambda))^{\rm eff}}$ such  that we can equivalently express \eqref{eq:velocityrhot} as $v^d_{j}(\lambda)={(\partial_\lambda e_{j}(\lambda))^{\rm eff}}/{(\partial_\lambda p_{j}(\lambda))^{\rm eff}}$. This formulation is used in a large portion of the GHD literature. 


In closing, we remark that, even though here we assumed the system to be in an eigenstate of the Hamiltonian, the TBA description can be used also for some (stationary) mixed states. This is true every time a generalized microcanonical representation applies \cite{Essler2016, Vidmar2016}. In essence, this means that the expectation values of all local observables in the mixed state can be reproduced, in the thermodynamic limit, by expectation values in a single, appropriately  chosen eigenstate of the Hamiltonian. For example, the densities corresponding to a generalized Gibbs state $\rho_{\rm GGE}\propto \exp[\sum_n \beta_{n} \CCharge]$ can be found minimising the ``generalized free energy" $f[\rho]= \sum_n \beta_{n} q_n[\rho]- s[\rho]$, which yields the following integral equations \cite{Yang1969}
\be
\log\eta_j(\lambda) \!\!= \!\!\sum_n \beta_n q_{n,j}(\lambda) \!+\! \sum_{k=1}^{N_s}\! \sigma_k T_{kj}\ast\log[1+\eta_k^{-1}](\lambda)\,,
\label{eq:GTBA}
\ee 
where we introduced the function
\be
\eta_j(\lambda)\equiv \frac{\rho^h_j(\lambda)}{\rho_j(\lambda)}=\frac{1}{\vartheta_j(\lambda)}-1.
\label{eq:etafun}
\ee
These equations, together with Eq.~\eqref{eq:TBT}, completely fix the densities of the generalized Gibbs state. Note that, if $\{\rho_j(\lambda)\}$ and $\{\rho^h_j(\lambda)\}$ solve  Eqs.~\eqref{eq:TBT} and  \eqref{eq:GTBA}, the generalized free energy can be written compactly as
\be
f = \frac{e_0}{T} - \sum_{k=1}^{N_s} \sigma_k \!\!\int_{-\Lambda}^{\Lambda} \!\!\!{\rm d}\lambda\,\, a_k(\lambda) \log\!\left[1+\frac{\rho_k(\lambda)}{\rho_k^h(\lambda)}\right]\!.
\label{eq:thermalfreeenergy}
\ee 
We also remark that the derivatives of $\log\eta_k(\lambda)$ with respect to the ``chemical potentials" $\beta_n$ are related to the dressed quantities. Indeed, comparing Eqs.~\eqref{eq:dressing1} and \eqref{eq:GTBA} we find ${\partial_{\beta_n}\!\!\log\eta_k(\lambda)=A(\Delta) \partial_\lambda q^d_{n-1,k}(s, \lambda)}$.
In order to find the explicit form of $q_{n,k}(\lambda)$, we use the explicit form of $q_{n,k}(\lambda)$ reported after Eq.~\eqref{eq:charge}.

\subsubsection{Drude weights from TBA}
\label{sec:DrudeTBA}

As an application of the TBA formalism, we here present  the calculation of certain Drude weights. We remark that, although these quantities are expressed in terms of dynamical correlations on {equilibrium states}, the calculation of generic Drude weights in Bethe-ansatz integrable models remained unfeasible for a long time. Indeed, correlation functions usually fall outside the compass of Bethe-ansatz techniques. In some cases, however, it has been possible to relate Drude weights to simple spectral or thermodynamic properties that can be efficiently determined using TBA. 
In particular, 
 we briefly review Zotos's calculations of the energy \cite{Zotos2016} and spin 
\cite{Zotos1999} Drude weights for the spin-1/2 XXZ chain with 
$\Delta=\cos(\pi/m)$ at finite temperature $T$. The results for the energy 
Drude weight are directly generalized to any $\Delta$ while those for the spin 
Drude have been extended to $\Delta=\cos(\pi \ell/m)$ with coprime integers $\ell$ and 
$m$ \cite{Urichuk2018} [see Sec.~\ref{sec:GHDDrude}  for a discussion].      

Let us begin by considering the case of the energy Drude weight, which, as we 
shall see, is considerably simpler. The crucial observation \cite{Zotos1997} is 
that in the spin-1/2 XXZ chain, the total energy current ${\JE=\sum_r 
j^{\rm (E)}_r}$ [see Eq.~\eqref{eq:jE}] is itself a conserved quantity. In 
particular, in our notation, $\JE$ coincides with $Q_2$ [see 
Eq.~\eqref{LocalCharges}]. This means that one can define a generalized Gibbs 
ensemble including such a current as a charge, i.e., $\rho_{GGE}\propto 
e^{-\beta H - \xi \JE}$, and compute its root densities following the 
last paragraph of the Sec.~\ref{sec:tba}. In particular, the free-energy 
density $f_\xi$ of this state takes the form \eqref{eq:thermalfreeenergy} where 
the densities of rapidities fulfill Eqs.~\eqref{eq:TBT} and \eqref{eq:GTBA} with  
$\beta_1=\beta$, $\beta_2=\xi$, and $\beta_{n\geq3}=0$. The Drude weight is then 
straightforwardly evaluated as [see  Eq.~\eqref{eq:DwC}]
\be
\Dwe=\frac{\beta^2}{2 L} \braket{(\JE)^2} = -\frac{\beta^3}{2}  \partial_\xi^2 f_\xi \big |_{\xi=0}\,.
\ee
This identity has been first used in \cite{Kluemper2002} to compute the energy 
Drude weight within the quantum transfer-matrix approach. 
The results are shown in Fig.~\ref{fig:drude_bethe}. 
Zotos, instead, found the 
explicit result from  TBA by combining Eqs.~\eqref{eq:TBT} and \eqref{eq:GTBA}. 
Using some straightforward identities among TBA functions [see, e.g., 
\cite{Urichuk2018}], the final expression can be written as 
\be
\Dwe=\frac{\beta^2 }{2} \sum_{k=1}^{N_s} \int_{-\Lambda}^{\Lambda} \!\!\!{\rm d}\lambda\,\ \!\!\! 
\frac{\rho_k^t(\lambda) (e_k^{\rm eff}(\lambda))^2 (v_k^d(\lambda))^2}{(1+\eta_k(\lambda))(1+\eta_k^{-1}(\lambda))}\,,
\label{eq:Drudeenergy}
\ee
where $e_k^{\rm eff}(\lambda)= 2\pi \sigma_k \rho^t_k(\lambda) A(\Delta)$ is the effective energy and $v_k^d(\lambda)$ the group velocity of the dressed excitations [cf. \eqref{eq:velocityrhot}]. The same method can be used to find higher cumulants of ${\cal J}^{(E)}$ \cite{Zotos2016, Urichuk2018}. 
   
\begin{figure}[t]
\begin{center}
%\includegraphics[width=0.90\linewidth]{figs_xxz/xxz_dwe_bethe.eps}
\includegraphics[width=0.90\linewidth]{xxz_dwe_bethe}
\caption{(Color online) Exact results for the energy Drude weight of the spin-1/2 XXZ
chain given in Eq.~(\ref{eq:XXZ-intro}) at zero magnetization. The data is taken from
\cite{Kluemper2002}.}
\label{fig:drude_bethe}
\end{center}
\end{figure}
 
The complication arising when considering the spin Drude weight is that the total spin current, as opposed to the total energy current, is not conserved. The calculation, however, can still be performed avoiding the explicit evaluation of correlation functions. The idea is to consider the system in a large finite volume $L$, to introduce a finite magnetic flux $L \phi$ through the chain, and to compute the Drude weight using the finite-$T$ Kohn formula \eqref{eq:Kohn}, i.e., in terms of the second derivative of the energy density with respect to the magnetic flux. The insertion of a magnetic flux can be easily treated in Bethe ansatz and results in a phase (``twist") $e^{i \phi L}$ multiplying the r.h.s.\ of \eqref{eq:BetheEquations}. For $L \phi$ finite in the thermodynamic limit (i.e., when $L \phi$ does not scale with the volume), the twist modifies the position of the rapidities of the strings only at sub-leading orders. This leads to 
\be
\lambda_{\alpha,L}^j(\phi)=\lambda_{\alpha,\infty}^j+\frac{g_{1,j}(\lambda_{\alpha,\infty}^j,\phi)}{L}+\frac{g_{2,j}(\lambda_{\alpha,\infty}^j,\phi)}{L^2}\,,
\label{eq:shiftedrapidities}
\ee
where we neglected $O(L^{-3})$ and introduced the subscripts $L/\infty$ to label rapidities in finite and infinite volume, respectively. The $\phi$-dependent functions $g_{1,j}(x,\phi)$ and $g_{2,j}(x,\phi)$ fulfill some integral equations determined through a $1/L$ expansion of the Bethe-Takahashi equations \eqref{eq:BetheTaka}. Plugging \eqref{eq:shiftedrapidities} into Eq.~\eqref{eq:energySH}, one can determine the second derivative of the energy density with respect to the twist in the thermodynamic limit and hence the Drude weight. This method has been introduced in \cite{Fujimoto1998} for the calculation of the charge Drude weight in the Fermi-Hubbard model and has been applied in \cite{Zotos1999} for the spin-1/2 XXZ chain. In the case of the XXZ chain, the result can be cast  into the following form 
\be
\Dws=\frac{\beta}{2} \sum_{k=1}^{N_s} \int_{-\Lambda}^{\Lambda} \!\!\!{\rm d}\lambda\,\ \!\!\! 
\frac{  \rho_k^t(\lambda) (n_k^{\rm eff}(\lambda))^2 (v_k^d(\lambda))^2}{(1+\eta_k(\lambda))(1+\eta_k^{-1}(\lambda))}\,,
\label{eq:Drudespin}
\ee  
where $n_k^{\rm eff}(\lambda)=2 \pi \sigma_k \rho_k^t(\lambda) \partial_\phi g_{1,k}(\lambda)$ fulfills the dressing equation \eqref{eq:dressing} by replacing $n_k^{\rm eff}(\lambda) \to q_k^{\rm eff}(\lambda)$ with driving $n_k$,  thus replacing $q_k(\lambda) $ by $n_k$ in Eq.~\eqref{eq:dressing} [cf. Eq.~\eqref{eq:strings} for the definition of the $n_k$]. 
The temperature dependence of $\Dws$ is illustrated in Fig.~\ref{fig:zotos99}.

As we will see in Sec.~\ref{sec:GHD},  GHD provides a general framework for computing Drude weights in TBA formalism. In particular, both Eq.~\eqref{eq:Drudeenergy} and Eq.~\eqref{eq:Drudespin} are
special cases of the generic GHD result Eq.~\eqref{eq:DrudeGHD}, which describes the Drude weights of all conserved charges.

\begin{figure}[t]
\begin{center}
%\includegraphics[width=0.90\linewidth]{figs_integrability/zotos99.eps}
\includegraphics[width=0.90\linewidth]{zotos99}
\caption{(Color online)
TBA results for the spin Drude weight $\Dws$ of the spin-1/2 XXZ chain versus $\Delta$ for different temperatures $T$ (measured in units of $J$) from \cite{Zotos1999}.
\label{fig:zotos99}}
\end{center}
\end{figure}



\subsection{Generalized hydrodynamics}
\label{sec:GHD}

The theory of generalized hydrodynamics concerns the evolution of integrable systems initially prepared in a state ${\rho}_0$ that is spatially inhomogeneous and then let to evolve unitarily with a homogeneous Hamiltonian. The main idea is that at large times, the expectation values of local observables become slowly varying functions of $x$ and $t$. This is much like the situation observed in the case of homogeneous quantum quenches [see, e.g., \cite{Essler2016, Eisert2015, Gogolin2016}]: initially the expectation values of local observables display fast oscillations but the latter dephase away for large times and expectation values become stationary even in the presence of a coherent unitary evolution. In the slow, late-time, regime, it is reasonable to expect that the expectation values can be described by a quasistationary state, namely 
\be\label{eq:hydrogen}
{\rm tr }\left[{\mathcal O}_x  e^{-i { H} t}   {\rho}_0 e^{i { H} t}\right]\overset{t\gg \tau_0}{\sim} {\rm tr }\left[{\mathcal O}_x   {\rho}_{\rm st}({x,t})\right],
\ee
where $H$ is the Hamiltonian of the system, ${\mathcal O}_x$ is a generic observable localized around the point $x$, ${\rho}_{\rm st}(x,t)$ is the density matrix describing the quasi-stationary state (retaining a slow space-time dependence), and $\tau_0$ is the time-scale for local relaxation. In general, the $x$-dependence in Eq.~\eqref{eq:hydrogen} is nontrivial for large but \emph{finite} times, while it is typically washed away at infinite times. 
Think, for example, of the free expansion of a gas released from a trap: the density of the gas vanishes at infinite times becoming trivially $x$ independent. There are some cases, however, where nontrivial effects of the problem's inhomogeneity persist even at infinite times. In that case, one can explicitly take the infinite-time limit of Eq.~\eqref{eq:hydrogen} turning it into an exact statement. An example is the so-called bipartitioning protocol where one suddenly joins together two systems that are initially in different stationary states (see Sec.~\ref{sec:bipartitioning}). 

A stationary state of the form  ${\rho}_{\rm st}(x,t)$ given by Eq.~\eqref{eq:hydrogen} has been termed \emph{locally quasi-stationary state} (LQSS) \cite{BertiniFagotti2016}. Specifically, based on the intuition developed for homogeneous quenches, it was argued that, at fixed $(x,t)$, the state ${\rho}_{\rm st}({x,t})$ is a generalized Gibbs state constructed with the charges of the Hamiltonian that controls the unitary time evolution. This means that ${\rho}_{\rm st}({x,t})$ is homogeneous, stationary, and admits a ``microcanonical'' representation in terms of a TBA representative eigenstate, or, equivalently, of a set of densities of rapidities $\{\rho_{k}(\lambda,x,t)\}$. Determining such space-time dependent functions is the central problem of the theory.  

A macroscopic number of constraints on these functions are obtained by considering the expectation values of the continuity equations of all local and quasilocal conserved charges from Eq.~\eqref{eq:higherconservations}, namely 
\be
\!\!\partial_t \dens_{x}(t) + \curr_{x}(t)-\curr_{x-1}(t)=0,\quad  x=1,\ldots,L,
\label{eq:continuity}
\ee
where $\dens_x$ is the density of charge $Q_n$ and $\curr_{x}$ its current.\footnote{We here simplify the notation introduced in Sec.~\ref{sec:theory} by writing $\curr_{x}$ instead of $j_x^{(Q_n)}$.} 
Here and in the following, we suppress the additional index $s$, keeping only the generic index $n$ for conserved charges. 
Assuming the validity of Eq.~\eqref{eq:hydrogen},  one obtains that, to leading order in time,  the expectation value of \eqref{eq:continuity} reads as  
\be
\partial_t {\rm tr }\left[\dens_{0}  {\rho}_{\rm st}({x,t})\right]+ \partial_x {\rm tr }\left[ \curr_{0}   {\rho}_{\rm st}({x,t})\right]=0\,.
\label{eq:evcontinuityleading}
\ee
The relevant time scale is the so-called Euler time, i.e., the  time scale at 
which the fastest quasiparticle excitations traverse a small fraction of a 
system's volume. We remark that this equation is already in the thermodynamic 
limit and, moreover, on its r.h.s., there are sub-leading corrections 
of $\mathcal{O}(t^{-b})$ with ${b>0}$. As shown in~\cite{Bertini2016,Castro-Alvaredo2016}, 
the constraint \eqref{eq:evcontinuityleading} is  sufficient  to fix the densities of 
rapidities to leading order in time. Specifically, 
Eq.~\eqref{eq:evcontinuityleading} is equivalent to the following continuity 
equation for the densities of rapidities
 \begin{equation}
  \partial_{t} \rho_{k}(\lambda, x,t)+  \partial_{x}(v^d_{k}(\lambda,x,t) \rho_{k}(\lambda, x,t)) = 0.
\label{eq:continuityrhoxt}  
\end{equation}
Here, $v^d_{k}(\lambda,x,t)$ is the group velocity of dressed excitations on the state ${\rho}_{\rm st}({x,t})$. The physical interpretation of this equation is straightforward: to leading order in time, the dynamics of $\{\rho_{k}(\lambda,x,t)\}$ can be described as if they were quasimomentum distributions for $N_s$ species of free classical particles moving in a density-dependent background. Indeed, the only effect of the interaction is a dressing of the group
velocity. These classical particles can be thought of as an ``asymptotic" version of the stable modes characterizing Bethe-ansatz integrable models. Indeed, for very large times and distances, the modes loose all phase information and behave like classical particles.  


The crucial step in passing from Eq.~\eqref{eq:evcontinuityleading} to Eq.~\eqref{eq:continuityrhoxt} makes use of the following expression for the expectation value of generic currents on the macrostate $\{\rho_{n}(\lambda)\}$  
\be
j^Q[\rho]=\sum_{k=1}^{N_s} \!\int \!\!{\rm d}\lambda\, q_k(\lambda) v^d_{k}(\lambda) \rho_k(\lambda),
\label{eq:current}
\ee
where $q_k(\lambda) $ is the bare charge of the associated density (c.f.\ Eq.~\eqref{eq:charge}). This form has been originally proposed for relativistic integrable quantum-field theories with diagonal scattering \cite{Castro-Alvaredo2016} --- through a crossing-symmetry argument  --- and for the spin-1/2 XXZ chain  \cite{Bertini2016} --- through a semiclassical argument. These arguments have been recently proven by an explicit resummation of form-factor\footnote{\label{ff:definition}In this context, the term ``form factor" indicates the matrix element of a local operator between two Hamiltonian eigenstates.} expansions \cite{Yoshimura2018, borsi2019current} in the aforementioned systems and by exact calculations in generic quadratic theories \cite{Fagotti:2017aa}. 

The form Eq.~\eqref{eq:current} is currently conjectured to apply to all Bethe-ansatz integrable models, including nested systems such as the Fermi-Hubbard model or the sine-Gordon quantum field theory, where one appropriately considers the contributions of all the species of rapidities. Even though an explicit proof of the general case is not yet available, Eq.~\eqref{eq:current} has been confirmed by numerical calculations, e.g., in the Fermi-Hubbard model \cite{Ilievski2017}. A rigorous derivation of Eq.~\eqref{eq:current} for spin-transport in the spin-1/2 XXZ chain has recently been accomplished in \textcite{Urichuk2018}. Finally, we remark that the form \eqref{eq:current} for the expectation values of currents has been shown to hold also for certain integrable classical field theories \cite{DoyonToda, Bastianello2018, Bulchandani2019, Cao_2019}.     



The simplification introduced by Eq.~\eqref{eq:continuityrhoxt} is remarkable: to determine the late-time properties of an integrable quantum many-body system, one does not need to solve the many-body Schr\"odinger equation but an immensely simpler system of differential equations. After discretizing the rapidity, these equations can be treated by standard methods for initial-value partial differential equations~
\cite{iFluid}, by ``characteristics"~\cite{Doyon2017b, Bulchandani2017} or by ``molecular dynamics"~\cite{FleaGas}, i.e., by simulating the dynamics of the classical gas whose rapidity distributions obey Eq.~\eqref{eq:continuityrhoxt}. There is, however, a remaining nontrivial step to make before a solution can be obtained: one has to
find the right initial conditions for $\{\rho_{k}(\lambda,x,t)\}$. This problem has not yet been solved for all initial states $\rho_0$ but only for a number of particular choices \cite{Bulchandani2017a,Bulchandani2017b, Doyon:2017aa, Caux2019}. Importantly, some of these choices give a good characterization of experimentally-accessible initial configurations. This has been explicitly demonstrated in~\cite{Schemmer}, where GHD has been argued to give the best available description of a cold atom experiment. 

Let us now focus on the most popular initial configuration accessible with GHD: the bipartitioning protocol, i.e., the time evolution of an initial state composed of the tensor product of two different homogeneous states $\rho_0\sim \rho_{\rm L}\otimes \rho_{\rm R}$ (see Sec.~\ref{sec:bipartitioning}). As mentioned before, since in this case, we can explicitly take the infinite-time limit, Eq.~\eqref{eq:continuityrhoxt} becomes exact. The solution is a function of the scaling variable $\zeta=x/t$, usually termed ``ray", and can be ``implicitly" written as \cite{Castro-Alvaredo2016, Bertini2016} 
\be
\!\!\vartheta_{k}(\lambda, \zeta)\!=\! [\eta^{\rm L}_{k}(\lambda)\!-\!\vartheta^{\rm R}_{k}(\lambda)]\, \Theta [v^d_{k}(\lambda,\zeta)- \zeta]\!+\!\vartheta^{\rm R}_{k}(\lambda),
\label{eq:continuitythetasol}   
\ee 
where $\Theta(x)$ is the step-function and $\vartheta_{k}^{\rm L/\rm R}(\lambda)$ characterize the homogeneous GGE emerging at infinite distance from the junction on the left and on the right, respectively.\footnote{We assumed that $\rho_{\rm L/R}$ have \emph{cluster decomposition properties}. Namely, they satisfy $\lim_{|x-y|\to\infty}\braket{O_1(x)O_2(y)}_{\rm L/R}=\braket{O_1(x)}_{\rm L/R} \braket{O_2(y)}_{\rm L/R}$ where the operators $O_i(x)$ are local (i.e, they act trivially far away from the site $x_i$) and $\braket{O(x)}_{\rm L/R} \equiv {\rm tr}[O(x)\rho_{\rm L/R}]$.} This solution is implicit because $v^d_{k}(\lambda,\zeta)$ depends itself on $\vartheta_{k}(\lambda, \zeta)$. The explicit result is obtained by formulating an initial guess for $v^d_{k}(\lambda,\zeta)$ and iterating Eqs.~\eqref{eq:continuitythetasol}, \eqref{eq:TBT}, and \eqref{eq:dressing} until convergence is reached (this is typically achieved in less than ten steps). This protocol has been used for studying nonlinear transport in integrable quantum many-body systems on the lattice \cite{Bertini2016, Piroli:2017aa, BertiniPiroli2018, DeLucaspintransport, ColluraAnalytic, BertiniPRL2018, Mazza2018, Eisler2019} as well as on the continuum \cite{Castro-Alvaredo2016, Mestyan2018, Bertini2019}. Moreover, it has also been used for analysing the dynamics of entanglement in inhomogeneous situations \cite{Bertini2018, Alba2019, Alba2018, Mestyan2019}. Next, in Sec.~\ref{sec:GHDDrude}, we will discuss how this protocol can be used for computing Drude weights. 

In concluding this brief review of GHD, we must mention that Eq.~\eqref{eq:continuityrhoxt} does not represent an end point: there are currently many ongoing efforts to extend its range of applicability. First of all, the equation furnishes only a leading-order-in-time characterization, or, more precisely, describes the system for large times $t$ and lengthscales $x \sim t$. In analogy with ordinary hydrodynamics, however, one would expect GHD to describe the asymptotic behavior of the system also on other lengthscales, for example, the diffusive one where $x\sim \sqrt{t}$. This can be achieved by finding the sub-leading corrections in $t$ to Eq.~\eqref{eq:continuityrhoxt}. In particular, in Sec.~\ref{sec:GHDDiffusion}, we will briefly discuss a correction, recently identified in \cite{DeNardisDiffusion}, which is able to describe diffusive behaviors. Currently, however, a systematic method to find all sub-leading corrections to Eq.~\eqref{eq:continuityrhoxt} has been devised only in the noninteracting case \cite{FagottiHigherGHD, Fagotti2019}. Another active research strand is to extend Eq.~\eqref{eq:continuityrhoxt} to the case in which the time evolution is determined by a spatially inhomogeneous Hamiltonian. In particular, \cite{DoyonYoshimura17} presented an extension valid in the case of a system confined to a slowly varying trapping potential, while \cite{Bastianello2019} considered the case of slowly varying Hamiltonian parameters. Finally, there are ongoing efforts to describe the evolution of the initial-state correlations under \eqref{eq:continuityrhoxt}~\cite{ruggiero2019quantum}. 




\subsubsection{GHD results for Drude weights}
\label{sec:GHDDrude}

Drude weights can be computed within GHD following two different approaches that, crucially, give coinciding results. Both approaches give access to the most general Drude weight 
\begin{align}
\Dw^{(n,m)}&= \frac{\beta}{2}\lim_{t\to\infty}\frac{1}{t}\sum_{r} \int_{-t/2}^{t/2}\!\!\!{\rm d}s \braket{\curr_{r}(s)\currm_{0}(0)}^{\rm c}\notag\\
&= \frac{\beta}{2}\lim_{t\to\infty}\sum_{r}{\rm Re}[\braket{\curr_{r}(t)\currm_{0}(0)}^{\rm c}],
\label{eq:GeneralDrude}
\end{align}
where $\braket{\cdot}^{\rm c}$ denotes the connected expectation value in a (grand-canonical) Gibbs Ensemble 
$\rho_{\rm GE}\propto \exp[-\beta H+ \sum_i \lambda_i O_i]$.  Here, the sum runs over all conserved U(1) charges $O_i$ of the system.
In Eq.~\eqref{eq:GeneralDrude}, $n$ and $m$ can label two different conserved charges. In the case $n=m$, one recovers the usual ``diagonal" Drude weight of the charge $\CCharge$. All results, however, can be directly extended to the case of expectation values in more general GGEs. Note that (i) in order to treat all charges on the same footing, we divided  the energy Drude weight by $\beta$ and (ii) the correlation function in \eqref{eq:GeneralDrude} is \emph{not} the Kubo correlation used in Eq.~\eqref{eq:Kubo}. 
In the limit $t\to\infty$, the two expressions, however, can be shown to coincide under mild assumptions \cite{Ilievski2013}.\footnote{Interestingly, for integrable models, $\lim_{t\to\infty}\sum_{r} \braket{\curr_{r}(t)\curr_{0}(0)}^{\rm c}$ turns out to be real. This implies that the Drude weight can also be defined using a ``asymmetric" integration, namely $\Dw^{(n,m)}=\frac{\beta}{2}\lim_{t\to\infty}\frac{1}{t}\sum_{r} \int_{0}^{t}{\rm d}s \braket{\curr_{r}(s)\currm_{0}(0)}^{\rm c}$.}

The first approach, proposed in~\cite{Ilievski2017a, Bulchandani2017b}, evaluates the Drude weight using the following formulation. One considers a bipartitioning protocol that connects two halves of the system (left ``L" and right ``R") initially prepared in the following different GGEs 
\be
\rho_{\rm GGE, L/R}\propto \exp[-\beta H+ \sum_i \mu_i N_i \pm (\beta_m/2) \CChargem]\,,
\ee
where $\CChargem$ is the $m$-th conserved charge of the system. In this setting, one can compute $\Dw^{(n,m)}$ as follows~\cite{Vasseur2015}
\be
\Dw^{(n,m)}=\lim_{\beta_m \to0}\lim_{t\to\infty} \frac{\beta}{2 t \beta_m} {{\rm tr}[{\curr_{0} e^{-i H t} \rho_{0} e^{i H t}}]},
\ee 
where $\rho_{0}\sim \rho_{\rm GGE, L}\otimes \rho_{\rm GGE, R}$.    
Using Eq.~\eqref{eq:current} one can express this relation in terms of TBA quantities as  
\be
\!\!\Dw^{(n,m)}\!\!=\! \frac{\beta}{2}\! \sum_{k=1}^{N_s} \!\int \!\!{\rm d}\zeta\!\!\int_{-\Lambda}^{\Lambda}\! \!\!\!\!\!{\rm d}\lambda\,q_{n,k}(\lambda) \frac{\partial [v^d_{k}(\lambda,\zeta) \rho_k(\lambda,\zeta)]}{\partial  \beta_m}\bigg |_{\beta_m=0},
\label{eq:DrudeDNI}
\ee
where $q_{n,k}(\lambda)$ are the bare charges corresponding to $\CCharge$. 

The second approach, introduced in \cite{DoyonSpohnDrude}, computes the Drude weight using ``hydrodynamic projections". The idea is to write the Drude weight in the form Eq.~\eqref{eq:GeneralDrude} and expand it in the basis of conserved charges (appropriately orthogonalised). More precisely, one views 
\be
\sum_{r}\braket{\curr_{r}(t)\curr_{0}(0)}^{\rm c} \equiv (\curr|\currm),
\ee
as a scalar product in the space of local operators and assumes that the only contributions surviving at infinite times are coming from the overlap with conserved-charge densities  
\be
\!\!\!\!\!\lim_{t\to\infty} (\curr|\currm) = \sum_{k,k'} (\curr |\densk) [\frak C^{-1}]_{k k'} (\denskp |\currm)
\label{eq:projection}
\ee 
where we defined $\frak C_{nm}=(\dens|\densm)$. This reasoning is similar in spirit to that leading to the Mazur bound but it is carried out directly in the thermodynamic limit. In general, this approach can be used to compute the asymptotic behavior (large $t$ large $x$) of dynamical correlation functions in generic inhomogeneous situations \cite{DoyonCorr17}.

The quantities appearing in Eq.~\eqref{eq:projection} are all directly computed within GHD and lead to the following final result
\be
\Dw^{(n,m)}\!\!= \frac{\beta}{2} \sum_{k=1}^{N_s} \!\int_{-\Lambda}^{\Lambda} \!\!\!\!\!{\rm d}\lambda\,\ \!\!\! 
\frac{  \rho_k^t(\lambda) (v_k^d(\lambda))^2 q_{n,k}^{\rm eff}(\lambda)q_{m,k}^{\rm eff}(\lambda)}{(1+\eta_k(\lambda))(1+\eta_k^{-1}(\lambda))}\!,
\label{eq:DrudeGHD}
\ee
where $v_k^d(\lambda)$ and $q_{m,k}^{\rm eff}(\lambda)$ are the group velocity of excitations and the effective charge in the Gibbs state, respectively (i.e., with densities of rapidities obtained from solving \eqref{eq:TBT} and \eqref{eq:GTBA} with all Lagrange multipliers vanishing but $\beta$ and $\mu$). Remarkably, as shown in \cite{DoyonSpohnDrude}, this expression agrees with that obtained from Eq.~\eqref{eq:DrudeDNI} if one plugs in the implicit solution \eqref{eq:continuitythetasol} of the GHD equation for the bibartitioning protocol and takes the derivative explicitly. 

Three generic features of Eq.~\eqref{eq:DrudeGHD} are: (i) it is symmetric under the exchange of $n$ and $m$, in accord with Onsager reciprocal relations; (ii) the Drude weight is obtained by summing up ``elementary Drude weights" (the integrand of \eqref{eq:DrudeGHD}) for each quasiparticle in the system; (iii) the Drude weight of a certain quantity vanishes when the associated effective charges vanish. This happens, for example, in the case of the spin transport in the spin-1/2 XXZ chain with $|\Delta|\geq1$ at zero magnetization  and for the charge transport in the Fermi-Hubbard model at half filling. 

The expression Eq.~\eqref{eq:DrudeGHD} holds for all TBA  solvable models. Its generalization to the nested case has been first reported in \cite{Ilievski2017} and, again, corresponds to a sum of elementary Drude weights for each type of quasiparticle in the system. In particular, we see that Eq.~\eqref{eq:DrudeGHD} agrees with the special cases \eqref{eq:Drudeenergy} and \eqref{eq:Drudespin} discussed in the previous section once one restores the trivial $\beta$ factor in the energy Drude weight. Moreover, the nested generalization of Eq.~\eqref{eq:DrudeGHD} reproduces the result of  \cite{Fujimoto1998} for the charge Drude weight in the Fermi-Hubbard model. This follows by a direct comparison between Eqs.~(5) and (7) of  \cite{Ilievski2017} and Eq.~(35) of \cite{Fujimoto1998}, nonetheless, to the best of our knowledge, it has not  been noticed  in the literature. The main point is to note that $\xi_c(k), \xi_{s k}(\lambda), \xi_{b k}(\lambda)$ in \cite{Fujimoto1998} are exactly the ``effective electron charges" for the Fermi-Hubbard chain [cf.\ Eqs.~(A46) in the supplemental material of \cite{Ilievski2017}]. In other words, they fulfill the nested generalization of the dressing equations~\eqref{eq:dressing} with driving terms respectively given by $\xi^0_c(k)=1, \xi^0_{s k}(\lambda)=0, \xi^0_{b k}(\lambda)=2k$ [cf. Eqs.~(15)--(17) and Eqs.~(29)--(31) in \cite{Fujimoto1998}].




\subsubsection{GHD results for diffusion constants}
\label{sec:GHDDiffusion}
 
In order to access the diffusive regime, one needs to identify the leading 
corrections to Eq.~\eqref{eq:evcontinuityleading}, going beyond the Euler scale. 
A scheme to achieve this goal --- based on  two main assumptions --- has been 
proposed in~\cite{DeNardisDiffusion} [see also \cite{DeNardis2018, 
Gopalakrishnan2018a, Gopalakrishnan2019}]. The first assumption is that for 
large $t$, the system can be characterised using hydrodynamics also on 
lengthscales $x\sim \sqrt{t}$. Namely, one assumes that local observables are 
still described by a slowly varying quasi-stationary state $\rho_{\rm st}(x,t)$. 
This state, however, cannot be interpreted as a space-time dependent GGE 
anymore, but it has contributions proportional to the spatial derivatives of the 
Lagrange multipliers. Under this assumption, Eq.~\eqref{eq:evcontinuityleading} 
continues to hold also to  the first sub-leading order. The expectation values of 
the currents, however, are no longer given by Eq.~\eqref{eq:current} and include 
corrections written in terms of spatial derivatives of the densities of 
rapidities. Specifically, they can be written as~\cite{DeNardis2018} 
\begin{align}
&{\rm tr }\left[ j_{n,0}   {\rho}_{\rm st}({x,t})\right]=\sum_{k=1}^{N_s} \!\int \!\!{\rm d}\lambda\, q_{n,k}(\lambda) v^d_{k}(\lambda) \rho_k(\lambda,x,t)\notag\\
&\,\,\,-\frac{1}{2}\!\!\int \!\!{\rm d}\lambda{\rm d}\mu\!\! \sum_{k,k'=1}^{N_s} \! q_{n,k}(\lambda) {\frak D}_{k,k'}(\lambda,\mu) \partial_x\rho_{k'}(\mu,x,t),
\label{eq:GHDcurrentdiffusive}
\end{align}
where the kernel ${\frak D}_{k,k'}(\lambda,\mu)$ depends on $\{\rho_k(\mu,x,t)\}$. This kernel is related to the diffusion (Onsager) matrix defined as\footnote{Note that \eqref{eq:Onsagermatrix} does not coincide with the Onsager matrix given in Eq.~\eqref{eq:Lad} as in the latter we used Kubo correlation functions. Once again, however, the two matrices can be shown to coincide under mild assumptions~\cite{Ilievski2013}.} 
\be
D_{n,m}\!=\!\sum_{r} \!\!\int_{-\infty}^\infty\!\!\!{\rm d}t \left( \braket{\curr_{r}(t) \currm_{0}(0)}^c-\frac{2}{\beta}\Dw^{(n,m)}\right)
\label{eq:Onsagermatrix}
\ee
as follows~\cite{DeNardisDiffusion} 
\be
\!\!\!\!\!D_{n,m}\!= \!\!\sum_{p} \!\!\int \!\!{\rm d}\lambda{\rm d}\mu\!\!\!\!\sum_{k,k'=1}^{N_s}\!\!\! q_{n,k}(\lambda) {\frak D}_{k,k'}(\lambda,\mu) q_{p,k'}(\lambda)  {\frak C}_{p,m}
\label{eq:OnsagerD}
\ee
where the first sum is over all the conserved charges of the system and the matrix ${\frak C}_{p,m}$ has been introduced below Eq.~\eqref{eq:projection}. Note that it is always possible to add a ``derivative term" $\propto o_{x}-o_{x-1}$ to a charge density (where $o_x$ is a local operator), without modifying the total charge. This introduces an ambiguity in the definition of charge densities beyond the leading order [see \cite{Fagotti2019} for more details]. In particular, the kernel ${\frak D}_{k,k'}(\lambda,\mu)$ depends on the specific choice of the densities of charges while the Onsager matrix is invariant~\cite{DeNardis2018}. The simple relation \eqref{eq:OnsagerD} is obtained by taking charges and currents to be scalar under $\mathcal{PT}$-symmetry~\cite{DeNardis2018}. Finally, we remark that corrections similar to Eq.~\eqref{eq:GHDcurrentdiffusive}, i.e., depending on the spatial derivatives of the densities of rapidities, appear in the expectation values of all local observables with kernels that are generically unknown.  

The explicit TBA expression for Eq.~\eqref{eq:Onsagermatrix} in models with a single species of quasiparticles has been determined in~\cite{DeNardisDiffusion} through an expansion in finite-temperature form factors (see the earlier footnote\textsuperscript{\ref{ff:definition}}).  In particular, it has been shown that Eq.~\eqref{eq:Onsagermatrix} is fully determined by form factors involving two particle-hole excitations. The expression for an arbitrary number of quasiparticles species has later been presented in~\cite{DeNardis2018} and reads as 
\begin{align}
D_{n,m}&\!=\!\int\!\frac{{\rm d}\mu_1{\rm d}\mu_2}{2}\!\!\!\sum_{k,k'=1}^{N_s}\!\! \biggl\{\!\frac{\rho^h_{k}(\mu_1)}{1+\eta_{k}(\mu_1)}\frac{\rho^h_{k'}(\mu_2)}{1+\eta_{k'}(\mu_2)}\notag\\
&\times\!\! \left(\frac{T^{\rm eff}_{k',k}(\mu_2,\mu_1) q^{\rm eff}_{n,k'}(\mu_2)}{\sigma_{k'} \rho^t_{k'}(\mu_2)}-\frac{T^{\rm eff}_{k,k'}(\mu_1,\mu_2) q^{\rm eff}_{n,k}(\mu_1)}{\sigma_k \rho^t_k(\mu_1)}\right)\notag\\
&\times\!\! \left(\frac{T^{\rm eff}_{k',k}(\mu_2,\mu_1) q^{\rm eff}_{m,k'}(\mu_2)}{\sigma_{k'} \rho^t_{k'}(\mu_2)}-\frac{T^{\rm eff}_{k,k'}(\mu_1,\mu_2) q^{\rm eff}_{m,k}(\mu_1)}{\sigma_k \rho^t_k(\mu_1)}\!\!\right)\notag\\
&\times  |v^d_{k}(\mu_1)- v^d_{k'}(\mu_2)|\biggr\}\,,
\label{eq:GHDDiffusion}
\end{align}
where both the effective charges $q^{\rm eff}_{n,k}(\lambda)$ and the ``effective scattering kernel" $T^{\rm eff}_{k,k'}(\lambda,\mu)$ fulfill \eqref{eq:dressing} with driving functions given by $q_{n,k}(\lambda)$ and $T_{k,k'}(\lambda-\mu)$ ($T^{\rm eff}_{k,k'}(\lambda,\mu)$ for fixed values of its ``second" arguments $k'$ and $\mu$), respectively. We note that, to obtain the result \eqref{eq:GHDDiffusion}, De Nardis, Bernard, and Doyon conjectured a general form for the kinematical poles for finite-density form factors: this represents the second main assumption of  \cite{DeNardisDiffusion}. 

Equation~\eqref{eq:GHDDiffusion} can be interpreted by realizing that, at the diffusive scale, the conserved modes of interacting integrable models, i.e., the quasiparticles, do not follow exactly free classical trajectories. As a consequence of the scattering, they perform a noisy motion around the classical trajectories with a variance that grows as $\sqrt{t}$. Such a noisy motion is responsible for the diffusive behavior~\cite{DeNardis2018, Gopalakrishnan2018a, Gopalakrishnan2019}. This simple argument can be refined to obtain a quantitative prediction in agreement with Eq.~\eqref{eq:GHDDiffusion} in the linear-response regime~\cite{Gopalakrishnan2018a}. Moreover, in accordance with this interpretation, Eq.~\eqref{eq:GHDDiffusion} vanishes for noninteracting models.

Including the ``diffusive correction" Eq.~\eqref{eq:GHDcurrentdiffusive} in the expectation value of the currents, the continuity equation for the space-time-dependent densities of rapidities takes the following Navier-Stokes form~\cite{DeNardisDiffusion} 
\begin{align}
 &\partial_{t} \rho_{k}(\lambda, x,t)+  \partial_{x}(v^d_{k}(\lambda,x,t) \rho_{k}(\lambda, x,t)) =\notag\\
 &+\frac{1}{2}\partial_x\left[\int \!\!{\rm d}\mu\! \sum_{k'=1}^{N_s} \! {\frak D}_{k,k'}(\lambda,\mu) \partial_x\rho_{k'}(\mu,x,t)\right]\!.
\label{eq:continuityrhoxtdiffusion} 
\end{align}
Of particular interest for this review is the case of the spin-1/2 XXZ chain with $|\Delta|>1$ for small perturbations around a zero-magnetization ($\magdens=0$) equilibrium state. In this case, Eq.~\eqref{eq:continuityrhoxtdiffusion} leads to the following heat-like equation for the profile $m(x,t)$ of the magnetization density~\cite{DeNardis2018}  
\begin{align}
\partial_{t} \magdens(x,t)= \DS \partial_x^2 \magdens(x,t)\,,
\end{align}
where the spin-diffusion constant is given by 
\be
\DS =\sum_{k=1}^{N_s} \int_{-\pi/2}^{\pi/2}\!{{\rm d}\mu} \frac{\rho^h_{k}(\mu)}{1+\eta_{k}(\mu)} |v^d_k(\mu)| \mathcal W_k^2,
\ee       
and the rapidity-independent coefficient $\mathcal W_k$ reads as  
\be
\mathcal W_k = \lim_{k'\to\infty}\frac{T^{\rm eff}_{k',k}(\mu,\lambda)}{\rho^t_{k'}(\mu)}\,.
\ee 









